Effective Minkowski Dimension of Deep Nonparametric Regression: Function Approximation and Statistical Theories

Existing theories on deep nonparametric regression have shown that when the input data lie on a low-dimensional manifold, deep neural networks can adapt to the intrinsic data structures. In real world applications, such an assumption of data lying exactly on a low dimensional manifold is stringent. This paper introduces a relaxed assumption that the input data are concentrated around a subset of $\mathbb{R}^d$ denoted by $\mathcal{S}$, and the intrinsic dimension of $\mathcal{S}$ can be characterized by a new complexity notation -- effective Minkowski dimension. We prove that, the sample complexity of deep nonparametric regression only depends on the effective Minkowski dimension of $\mathcal{S}$ denoted by $p$. We further illustrate our theoretical findings by considering nonparametric regression with an anisotropic Gaussian random design $N(0,\Sigma)$, where $\Sigma$ is full rank. When the eigenvalues of $\Sigma$ have an exponential or polynomial decay, the effective Minkowski dimension of such an Gaussian random design is $p=\mathcal{O}(\sqrt{\log n})$ or $p=\mathcal{O}(n^\gamma)$, respectively, where $n$ is the sample size and $\gamma\in(0,1)$ is a small constant depending on the polynomial decay rate. Our theory shows that, when the manifold assumption does not hold, deep neural networks can still adapt to the effective Minkowski dimension of the data, and circumvent the curse of the ambient dimensionality for moderate sample sizes.

==> adaptive_regression <==
\begin{thebibliography}{37}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\expandafter\ifx\csname url\endcsname\relax
  \def\url#1{\texttt{#1}}\fi
\expandafter\ifx\csname urlprefix\endcsname\relax\def\urlprefix{}\fi

\bibitem[{Altman(1992)}]{altman1992introduction}
\textsc{Altman, N.~S.} (1992).
\newblock An introduction to kernel and nearest-neighbor nonparametric
  regression.
\newblock \textit{The American Statistician}.

\bibitem[{Anderson(1962)}]{anderson1962introduction}
\textsc{Anderson, T.~W.} (1962).
\newblock An introduction to multivariate statistical analysis.

\bibitem[{Bahdanau et~al.(2014)Bahdanau, Cho and Bengio}]{bahdanau2014neural}
\textsc{Bahdanau, D.}, \textsc{Cho, K.} and \textsc{Bengio, Y.} (2014).
\newblock Neural machine translation by jointly learning to align and
  translate.
\newblock \textit{arXiv preprint arXiv:1409.0473}.

\bibitem[{Bickel and Li(2007)}]{BickelLi}
\textsc{Bickel, P.~J.} and \textsc{Li, B.} (2007).
\newblock Local polynomial regression on unknown manifolds.
\newblock \textit{Lecture Notes-Monograph Series}, \textbf{54} 177--186.

\bibitem[{Chatfield(2018)}]{chatfield2018introduction}
\textsc{Chatfield, C.} (2018).
\newblock \textit{Introduction to multivariate analysis}.
\newblock Routledge.

\bibitem[{Chen et~al.(2019)Chen, Jiang, Liao and Zhao}]{chen2019efficient}
\textsc{Chen, M.}, \textsc{Jiang, H.}, \textsc{Liao, W.} and \textsc{Zhao, T.}
  (2019).
\newblock Efficient approximation of deep relu networks for functions on low
  dimensional manifolds.
\newblock \textit{Advances in neural information processing systems},
  \textbf{32}.

\bibitem[{Chen et~al.(2022)Chen, Jiang, Liao and Zhao}]{chen2022nonparametric}
\textsc{Chen, M.}, \textsc{Jiang, H.}, \textsc{Liao, W.} and \textsc{Zhao, T.}
  (2022).
\newblock Nonparametric regression on low-dimensional manifolds using deep relu
  networks: Function approximation and statistical recovery.
\newblock \textit{Information and Inference: A Journal of the IMA}, \textbf{11}
  1203--1253.

\bibitem[{Cheng and Wu(2013)}]{cheng2012local}
\textsc{Cheng, M.-Y.} and \textsc{Wu, H.-t.} (2013).
\newblock Local linear regression on manifolds and its geometric
  interpretation.
\newblock \textit{J. Amer. Statist. Assoc.}, \textbf{108} 1421--1434.

\bibitem[{Cloninger and Klock(2020)}]{cloninger2020relu}
\textsc{Cloninger, A.} and \textsc{Klock, T.} (2020).
\newblock Relu nets adapt to intrinsic dimensionality beyond the target domain.
\newblock \textit{arXiv preprint arXiv:2008.02545}.

\bibitem[{Ellis and Maitra(2007)}]{ellis2007multivariate}
\textsc{Ellis, N.} and \textsc{Maitra, R.} (2007).
\newblock Multivariate gaussian simulation outside arbitrary ellipsoids.
\newblock \textit{Journal of Computational and Graphical Statistics},
  \textbf{16} 692--708.

\bibitem[{Fan and Gijbels(1996)}]{fan1996local}
\textsc{Fan, J.} and \textsc{Gijbels, I.} (1996).
\newblock \textit{Local Polynomial Modelling and Its Applications}.
\newblock Monographs on statistics and applied probability series, Chapman \&
  Hall.

\bibitem[{Federer(1959)}]{federer1959curvature}
\textsc{Federer, H.} (1959).
\newblock Curvature measures.
\newblock \textit{Transactions of the American Mathematical Society},
  \textbf{93} 418--491.

\bibitem[{Goodfellow et~al.(2014)Goodfellow, Pouget-Abadie, Mirza, Xu,
  Warde-Farley, Ozair, Courville and Bengio}]{goodfellow2014generative}
\textsc{Goodfellow, I.}, \textsc{Pouget-Abadie, J.}, \textsc{Mirza, M.},
  \textsc{Xu, B.}, \textsc{Warde-Farley, D.}, \textsc{Ozair, S.},
  \textsc{Courville, A.} and \textsc{Bengio, Y.} (2014).
\newblock Generative adversarial nets.
\newblock In \textit{Advances in neural information processing systems}.

\bibitem[{Grassberger and Procaccia(1983)}]{grassberger1983measuring}
\textsc{Grassberger, P.} and \textsc{Procaccia, I.} (1983).
\newblock Measuring the strangeness of strange attractors.
\newblock \textit{Physica D: nonlinear phenomena}, \textbf{9} 189--208.

\bibitem[{Graves et~al.(2013)Graves, Mohamed and Hinton}]{graves2013speech}
\textsc{Graves, A.}, \textsc{Mohamed, A.-r.} and \textsc{Hinton, G.} (2013).
\newblock Speech recognition with deep recurrent neural networks.
\newblock In \textit{2013 IEEE international conference on acoustics, speech
  and signal processing}. IEEE.

\bibitem[{Gu et~al.(2017)Gu, Holly, Lillicrap and Levine}]{gu2017deep}
\textsc{Gu, S.}, \textsc{Holly, E.}, \textsc{Lillicrap, T.} and \textsc{Levine,
  S.} (2017).
\newblock Deep reinforcement learning for robotic manipulation with
  asynchronous off-policy updates.
\newblock In \textit{2017 IEEE international conference on robotics and
  automation (ICRA)}. IEEE.

\bibitem[{Gy{\"o}rfi et~al.(2006)Gy{\"o}rfi, Kohler, Krzyzak and
  Walk}]{gyorfi2006distribution}
\textsc{Gy{\"o}rfi, L.}, \textsc{Kohler, M.}, \textsc{Krzyzak, A.} and
  \textsc{Walk, H.} (2006).
\newblock \textit{A distribution-free theory of nonparametric regression}.
\newblock Springer Science \& Business Media.

\bibitem[{Hu et~al.(2018)Hu, Shen and Sun}]{hu2018squeeze}
\textsc{Hu, J.}, \textsc{Shen, L.} and \textsc{Sun, G.} (2018).
\newblock Squeeze-and-excitation networks.
\newblock In \textit{Proceedings of the IEEE conference on computer vision and
  pattern recognition}.

\bibitem[{Kpotufe(2011)}]{NIPS2011_4455}
\textsc{Kpotufe, S.} (2011).
\newblock $k$-{NN} regression adapts to local intrinsic dimension.
\newblock In \textit{Advances in Neural Information Processing Systems 24}
  (J.~Shawe-Taylor, R.~S. Zemel, P.~L. Bartlett, F.~Pereira and K.~Q.
  Weinberger, eds.). 729--737.

\bibitem[{Kpotufe and Garg(2013)}]{NIPS2013_5103}
\textsc{Kpotufe, S.} and \textsc{Garg, V.~K.} (2013).
\newblock Adaptivity to local smoothness and dimension in kernel regression.
\newblock In \textit{Advances in Neural Information Processing Systems 26}
  (C.~J.~C. Burges, L.~Bottou, M.~Welling, Z.~Ghahramani and K.~Q. Weinberger,
  eds.). 3075--3083.

\bibitem[{Krizhevsky et~al.(2012)Krizhevsky, Sutskever and
  Hinton}]{krizhevsky2012imagenet}
\textsc{Krizhevsky, A.}, \textsc{Sutskever, I.} and \textsc{Hinton, G.~E.}
  (2012).
\newblock Imagenet classification with deep convolutional neural networks.
\newblock In \textit{Advances in neural information processing systems}.

\bibitem[{Levina and Bickel(2004)}]{levina2004maximum}
\textsc{Levina, E.} and \textsc{Bickel, P.} (2004).
\newblock Maximum likelihood estimation of intrinsic dimension.
\newblock \textit{Advances in neural information processing systems},
  \textbf{17}.

\bibitem[{Liao et~al.(2021)Liao, Maggioni and Vigogna}]{liao2021multiscale}
\textsc{Liao, W.}, \textsc{Maggioni, M.} and \textsc{Vigogna, S.} (2021).
\newblock Multiscale regression on unknown manifolds.
\newblock \textit{arXiv preprint arXiv:2101.05119}.

\bibitem[{Liu et~al.(2021)Liu, Chen, Zhao and Liao}]{liu2021besov}
\textsc{Liu, H.}, \textsc{Chen, M.}, \textsc{Zhao, T.} and \textsc{Liao, W.}
  (2021).
\newblock Besov function approximation and binary classification on
  low-dimensional manifolds using convolutional residual networks.
\newblock In \textit{International Conference on Machine Learning}. PMLR.

\bibitem[{Long et~al.(2015)Long, Shelhamer and Darrell}]{Long_2015_CVPR}
\textsc{Long, J.}, \textsc{Shelhamer, E.} and \textsc{Darrell, T.} (2015).
\newblock Fully convolutional networks for semantic segmentation.
\newblock In \textit{The IEEE Conference on Computer Vision and Pattern
  Recognition (CVPR)}.

\bibitem[{Muller and Stewart(2006)}]{muller2006linear}
\textsc{Muller, K.~E.} and \textsc{Stewart, P.~W.} (2006).
\newblock \textit{Linear model theory: univariate, multivariate, and mixed
  models}.
\newblock John Wiley \& Sons.

\bibitem[{Nakada and Imaizumi(2020)}]{nakada2020adaptive}
\textsc{Nakada, R.} and \textsc{Imaizumi, M.} (2020).
\newblock Adaptive approximation and generalization of deep neural network with
  intrinsic dimensionality.
\newblock \textit{J. Mach. Learn. Res.}, \textbf{21} 1--38.

\bibitem[{Pakman and Paninski(2014)}]{pakman2014exact}
\textsc{Pakman, A.} and \textsc{Paninski, L.} (2014).
\newblock Exact hamiltonian monte carlo for truncated multivariate gaussians.
\newblock \textit{Journal of Computational and Graphical Statistics},
  \textbf{23} 518--542.

\bibitem[{Panayotov et~al.(2015)Panayotov, Chen, Povey and
  Khudanpur}]{panayotov2015librispeech}
\textsc{Panayotov, V.}, \textsc{Chen, G.}, \textsc{Povey, D.} and
  \textsc{Khudanpur, S.} (2015).
\newblock Librispeech: an asr corpus based on public domain audio books.
\newblock In \textit{2015 IEEE International Conference on Acoustics, Speech
  and Signal Processing (ICASSP)}. IEEE.

\bibitem[{Petersen and Voigtlaender(2018)}]{PETERSEN2018296}
\textsc{Petersen, P.} and \textsc{Voigtlaender, F.} (2018).
\newblock Optimal approximation of piecewise smooth functions using deep relu
  neural networks.
\newblock \textit{Neural Networks}, \textbf{108} 296--330.

\bibitem[{Pope et~al.(2021)Pope, Zhu, Abdelkader, Goldblum and
  Goldstein}]{pope2021intrinsic}
\textsc{Pope, P.}, \textsc{Zhu, C.}, \textsc{Abdelkader, A.}, \textsc{Goldblum,
  M.} and \textsc{Goldstein, T.} (2021).
\newblock The intrinsic dimension of images and its impact on learning.
\newblock \textit{arXiv preprint arXiv:2104.08894}.

\bibitem[{Schmidt-Hieber(2019)}]{schmidt2019deep}
\textsc{Schmidt-Hieber, J.} (2019).
\newblock Deep relu network approximation of functions on a manifold.
\newblock \textit{arXiv preprint arXiv:1908.00695}.

\bibitem[{Tsybakov(2008)}]{tsybakov2008introduction}
\textsc{Tsybakov, A.~B.} (2008).
\newblock \textit{Introduction to Nonparametric Estimation}.
\newblock 1st ed. Springer Publishing Company, Incorporated.

\bibitem[{Wahba(1990)}]{wahba1990spline}
\textsc{Wahba, G.} (1990).
\newblock \textit{Spline models for observational data}, vol.~59.
\newblock Siam.

\bibitem[{Yang et~al.(2015)Yang, Tokdar et~al.}]{yang2015minimax}
\textsc{Yang, Y.}, \textsc{Tokdar, S.~T.} \textsc{et~al.} (2015).
\newblock Minimax-optimal nonparametric regression in high dimensions.
\newblock \textit{Ann. Statist.}, \textbf{43} 652--674.

\bibitem[{Yarotsky(2017)}]{YAROTSKY2017103}
\textsc{Yarotsky, D.} (2017).
\newblock Error bounds for approximations with deep relu networks.
\newblock \textit{Neural Networks}, \textbf{94} 103--114.

\bibitem[{Young et~al.(2018)Young, Hazarika, Poria and
  Cambria}]{young2018recent}
\textsc{Young, T.}, \textsc{Hazarika, D.}, \textsc{Poria, S.} and
  \textsc{Cambria, E.} (2018).
\newblock Recent trends in deep learning based natural language processing.
\newblock \textit{ieee Computational intelligenCe magazine}, \textbf{13}
  55--75.

\end{thebibliography}

